CORSD: Class-Oriented Relational Self Distillation

Knowledge distillation conducts an effective model compression method while holding some limitations:(1) the feature based distillation methods only focus on distilling the feature map but are lack of transferring the relation of data examples; (2) the relational distillation methods are either limited to the handcrafted functions for relation extraction, such as L2 norm, or weak in inter- and intra- class relation modeling. Besides, the feature divergence of heterogeneous teacher-student architectures may lead to inaccurate relational knowledge transferring. In this work, we propose a novel training framework named Class-Oriented Relational Self Distillation (CORSD) to address the limitations. The trainable relation networks are designed to extract relation of structured data input, and they enable the whole model to better classify samples by transferring the relational knowledge from the deepest layer of the model to shallow layers. Besides, auxiliary classifiers are proposed to make relation networks capture class-oriented relation that benefits classification task. Experiments demonstrate that CORSD achieves remarkable improvements. Compared to baseline, 3.8%, 1.5% and 4.5% averaged accuracy boost can be observed on CIFAR100, ImageNet and CUB-200-2011, respectively.

==> chapters/discussions.tex <==
\section{Discussions}
\subsection{Visualization}
%\paragraph{Visualization} 
%In order to have a better understanding of the effectiveness of inter-class and intra-class relation capturing of TORSD, we visualize the distributions of samples in feature space at different depths.
%The distribution visualization can help for interpretability of TORSD in a straight-forward manner.
%As depicted in Figure~\ref{fig:3}, t-SNE visualizations~\cite{tSNE} with ResNeXt101-8 trained on CIFAR100 are conducted. We can make
%the following observations: (a) From each row of Figure~\ref{fig:3}, the deeper feature map is, the more compact clusters are. It proves that the relation of data samples is more salient in deeper layers. Concretely, the distances within the positive pairs (intra-class) are close while the negative pairs (inter-class) tend to distribute without intersection or wide of mark. (b) Compared with baseline, the ability of deep neural network at each depth to concentrate features is significantly improved with the relation distillation. It indicates that our relation distillation can help network to obtain more high-level semantic relation of samples in feature maps, especially for shallow layers.
%(c) When we further add the auxiliary classifiers, the performance of clustering in feature space are much more remarkable, which can help the deep neural network to better classify samples. It indicates that our proposed auxiliary classifiers can help the relation networks to capture task-oriented relation which is essential for classification task.


In order to have a better understanding of the enhancement of inter-class and intra-class relation of TORSD, we visualize the distributions of samples in feature space at different depths.
%The distribution visualization can help for interpretability of TORSD in a straight-forward manner.
As depicted in Figure~\ref{fig:3}, t-SNE visualizations~\cite{tSNE} with ResNeXt101-8 trained on CIFAR100 are conducted. 
%We can make the following observations: (a) From each row of Figure~\ref{fig:3}, the deeper feature map is, the more compact clusters are. It proves that the relation of data samples is more salient in deeper layers. Concretely, the distances within the positive pairs (intra-class) are close while the negative pairs (inter-class) tend to distribute without intersection or wide of mark. (b) Compared with baseline, the ability of deep neural network at each depth to concentrate features is significantly improved with the relation distillation. It indicates that our relation distillation can help network to obtain more high-level semantic relation of samples in feature maps, especially for shallow layers.
%(c) When we further add the auxiliary classifiers, the performance of clustering in feature space are much more remarkable, which can help the deep neural network to better classify samples. It indicates that our proposed auxiliary classifiers can help the relation networks to capture task-oriented relation which is essential for classification task.
When we successively add relation network training and auxiliary classifier training to the baseline, the performance of each block to cluster samples in feature space are much more remarkable, which can help the deep neural network to better classify samples.

%\paragraph{Sorted Separability} In Table~\ref{5}, we further calculate the sorted separability at each depth.
%Here we use SSE/SSB to evaluate the distinct capability of the model, SSE stands for sum of squared error while SSB is short for sum of squares between groups. Note that a smaller SSE/SSB indicates the feature space is denser. It can be observed that: (a) The SSE/SSB decreases as depth gets deeper. (b) The SSE/SSB decreases as our proposed techniques superimpose over one another. In summary, with our proposed TORSD, the model can obtain more separable feature space at different depths, and thus achieves higher classification accuracy.

\subsection{Ablation Study and Sensitivity Study}\label{sec:ablation}
\paragraph{Ablation Study} As shown in Table~\ref{6}, an ablation study on CIFAR100 with ResNet18 has been conducted to demonstrate the individual effectiveness of the proposed losses in TORSD. It can be observed that each loss in our method has its individual effectiveness and they can be utilized together to achieve better performance. Note that due to the specific role of each loss in our TORSD, we stack the losses one by one in a logical way to show the effectiveness of each loss, rather than randomly combining losses or individually studying on $\mathcal{L}_{RD}$, $\mathcal{L}_{NAC}$ or $\mathcal{L}_{PAC}$ without other necessary losses.



%Therefore, both randomly combining losses and only studying on $\mathcal{L}_{RD}$ or $\mathcal{L}_{NAC}$ or $\mathcal{L}_{PAC}$ without other necessary losses do not make much sense.
\paragraph{Sensitivity Study} 
% Six hyper-parameters are introduced to balance different losses in our TORSD. 
The sensitivity study of each hyper-parameter with ResNet18 on CIFAR100 are shown in Figure~\ref{fig:hyper}. Since the values of different losses vary in one order of magnitude at most, the values of hyper-parameters for different losses differ from $10^{-1}$ to $10^{-2}$ for the loss balancing. It can be observed that for the worst hyper-parameter setting case, it only leads to a 0.57\% accuracy drop compared with the best hyper-parameter setting, which is still 1.91\% higher than SD and 3.46\% higher than baseline, indicating that our method is robust to the choice of hyper-parameters.
\input{tabs/loss_study}

==> chapters/intro.tex <==
\section{Introduction}

Driven by deep neural networks (DNNs), natural language processing %~\cite{Authors01,Authors02,Authors03,Alpher01}
~\cite{Authors02}
and computer vision
%~\cite{Alpher02,Alpher03,Alpher04} 
~\cite{Alpher09,Alpher03} 
have been developing at an unprecedented speed. The success of state-of-the-art (SOTA) models rely on a high cost of computation and memory, and various kinds of techniques have been proposed for model compression, such as pruning
%~\cite{Authors04,Authors05}, 
~\cite{Authors04},
quantization
%~\cite{Alpher05,Alpher06} 
~\cite{Alpher06} 
and knowledge distillation 
%~\cite{Author06,Author07,Author08,Author09,Author10}. 
~\cite{Author08,Author10}. 
Knowledge distillation can be seen as a compression method which is inspired by knowledge transferring from a teacher model to a student model. Since the student is trained to mimic the logits or features of the teacher, the student can inherit the dark knowledge from the teacher, and thus achieving better performance. 
Moreover, self distillation~\cite{Author11} (SD) has been proposed to distill knowledge from deeper layers to shallower layers within a model. Due to its simplicity and effectiveness, SD has become a kind of technique widely used for both model compression and model accuracy boosting.

Recently, relation learning has become increasingly
popular in computer vision tasks, such as object detection~\cite{RNDetection} and video question answering~\cite{RNVideo}. This technique can help capture the relation between pixels, frames or data samples which is also of great value for relational knowledge distillation~\cite{Alpher07}. However in the field of knowledge distillation, most of the methods with or without relation learning including SD,
are faced of the following two issues:
(1) Previous methods without relation learning only focus on the alignment of output logits~\cite{Author10} or features
%~\cite{Alpher04,Alpher01,Alpher17,Alpher18,Author24} 
~\cite{Alpher17,Alpher18} 
from teacher to student but ignore the transferring of relations of data examples. As a result, these knowledge distillation methods only transfer the individual information rather than structured knowledge that is valuable for the task, leading to low-efficiency distillation;
(2) Lately, some works propose to improve the performance of knowledge distillation by transferring relation of data samples but are limited in
handcrafted functions for relation calculation, such as $L_{2}$ norm~\cite{Alpher07}
or inner product~\cite{Author18}. These naive relation calculation methods 
often fail to make full use of the relational knowledge of inter-class contrastiveness and intra-class similarity, and the
direct transferring of the knowledge from teacher to student ignores the hierarchical feature divergence within the model.

In this work, we propose a novel training framework named Task-Oriented Relational Self Distillation (TORSD) to overcome these obstacles. 
In order to make full use of sample relations,
we use structured input where each input image is randomly coupled with a positive image of the same class and a negative image of a different class. Rather than using handcrafted functions for relation calculation, we design the trainable relation networks to capture the inter-class and intra-class relation information of the structured input and then distill this relational knowledge from the deepest layer to shallow layers within a deep neural network.

%%%%%%Concretely, the proposed relation networks, which consist of a feature projection layer with several convolutional layers and a pooling layer, along with a Relational Interaction Block (RIB), are attached to different depths of the backbone to capture relations.
Concretely, the proposed relation networks, which consist of a Feature Projection Layer (FPL) and a Relational Interaction Block (RIB), are attached to different depths of the backbone to capture relation. 
FPL is utilized for feature projection of structured input, and RIB is designed to calculate the relation within the projected features. 
As the shallow layers encode more low-level features while more high-level semantic features can be extracted by the deep layers, the relation networks at each depth are independent.
With the relation networks, the structured relation of data examples can be well extracted, and this can be regarded as a distance measure in the projected feature space.

%%%%%%In order to train the relation networks for better relation modeling and reinforcement, we adopt the typical technique triplet loss in metric learning~\cite{Author26}, where the original $L_2$ norm is replaced with our proposed RIB as the adaptive distance metric for relation extraction.
In order to train the relation networks for better relation modeling and reinforcement, we adopt the typical technique triplet loss in metric learning~\cite{Author26} to further enhance the inter-class contrastiveness and intra-class similarity. As a result, the class-aware relation is obtained and enhanced, and then be transferred from the deepest layer to shallow layers.
And the whole deep neural network can better discriminate and classify samples.
Comparing TORSD to previous relational knowledge distillation method RKD~\cite{Alpher07}, the intra-class distances in feature space are more closely interrelated while the inter-class distances are magnified.

%%%%%%Moreover, auxiliary classifiers are proposed to help relation networks to capture task-oriented relations that are beneficial to classification tasks. Specifically, the relation networks in TORSD are not only trained with triplet loss but also trained with auxiliary task loss which performs the same task as the whole neural network does. Therefore, by transferring these task-oriented relational knowledge, the deep neural network can not only achieve the alignment of captured relations, but also enhance all the layers, especially for shallow layers, to considerably generate more valuable features which are essential for classification.
Moreover, auxiliary classifiers are proposed to help relation networks to capture task-oriented relation that are beneficial to classification task. Specifically, FPL in relation network is trained by auxiliary classifier with auxiliary task loss which performs the same task as the whole neural network does. In this way, more valuable features in projected features which are essential for classification are generated, and thus the relation extracted by RIB can be more task-oriented.


Since the relation networks, auxiliary classifiers and proposed losses in our method are only required in the training period, our method does not introduce any additional computation or memory overheads during inference. 
%%%%%%An overview results on CIFAR100 is shown in Figure~\ref{fig:results_overview}. Without bells and whistles, our proposed TORSD achieves excellent improvements compared with baseline, where a 4.74$\%$ accuracy boost can be observed on average across all models. Also, extensive experiments demonstrate that the proposed TORSD achieves a consistent and significant accuracy boost across various neural networks and datasets. We have also conducted detailed feature map visualization, ablation study and sensitivity study for better understanding of TORSD. To sum up, the contribution of this work can be summarized as follows:
Extensive experiments demonstrate that the proposed TORSD achieves a consistent and significant accuracy boost across various neural networks and datasets. We have also conducted detailed feature map visualization, ablation study and sensitivity study for better understanding of TORSD. To sum up, the contribution of this work can be summarized as follows:

\begin{itemize}
 \item We propose a novel training framework named TORSD. The trainable relation networks are designed to capture inter-class and intra-class relations of structured input, and the transferring of the relational knowledge from the deepest layer to shallow layers enables the whole network to better discriminate and classify input.
 \item Auxiliary classifiers are utilized to help the relation networks for task-oriented relation extraction from the projected features that are beneficial to classification task, leading to high-efficiency relational distillation.
 \item Extensive experiments on three datasets across six neural networks demonstrate that our proposed TORSD outperforms the state-of-the-art distillation methods by a large margin. On average, 1.93$\%$, 4.74$\%$, 1.44$\%$ and 4.42$\%$ accuracy boost can be observed on CIFAR10, CIFAR100, ImageNet and CUB-200-2011, respectively.
\end{itemize}
\input{images/framework}

==> chapters/related_works.tex <==
\section{Related Works}
% \subsection{Knowledge Distillation}
%%%%%%Knowledge distillation is one of the most effective methods for model compression and acceleration. Breiman and Shang~\shortcite{Author12} first propose to train a single tree model to approximate the performance of multiple tree models which is also of better interpretability.
%%%%%%Based on this method, Bucila \textit{et al.}~\shortcite{Alpher08} first exploit the idea of employing the large ensemble models to train a neural network. Hinton \textit{et al.}~\cite{Author10} further propose the concept of knowledge distillation and introduce a hyper-parameter, temperature, to control the training of student models. FitNet~\cite{Author08} is put forward with the concept of hint learning to reduce the distance between feature maps of students and teachers. Many subsequent works have presented various approaches in various applications for knowledge distillation. Shen \textit{et al.}~\shortcite{Author13} combine adversarial learning with knowledge distillation
%%%%%%to minimize the differences between features of students and teachers. Zagoruyko \textit{et al.}~\shortcite{Author09} apply feature distillation on the attention map of neural networks across different layers to achieve higher accuracy. Aside from image classification, many works have been proposed to explore knowledge distillation in tasks such as object detection~\cite{FGFI,OverhaulFD,FKD}, semantic segmentation~\cite{SKD}, face recognition~\cite{FaceKD}, pretrained language model~\cite{DistillBERT,BERTDistill} and model robustness~\cite{AuxiliaryTrain}, just name a few.
% \paragraph{Knowledge Distillation}
Knowledge distillation is one of the most effective methods for model compression and acceleration. Breiman and Shang~\shortcite{Author12} first propose to train a single tree model to approximate the performance of multiple tree models.
Based on this method, Hinton \textit{et al.}~\cite{Author10} further propose the concept of knowledge distillation, known as teacher-student distillation and introduce a hyper-parameter, temperature, to control the training of student models. Many subsequent works have presented various approaches for knowledge distillation. FitNet~\cite{Author08} is put forward with the concept of hint learning to reduce the distance between feature maps of students and teachers. 
Shen \textit{et al.}~\shortcite{Author13} combine adversarial learning with knowledge distillation to minimize the differences between features of students and teachers. Zagoruyko \textit{et al.}~\shortcite{Author09} apply feature distillation on the attention map of neural networks across different layers to achieve higher accuracy. 

% \subsection{Self Distillation}
\paragraph{Self Distillation}

Recently, a number of works~\cite{Author14,BornAgain,Author16} have shown that distilling a teacher model into a student model of identical architecture can improve the student performance to even surpass the teacher. The idea of self distillation first comes from Zhang \textit{et al.}~\shortcite{Author11}, where a one-step self distillation framework is proposed. 
The key point is to transfer the knowledge from deep layers to the shallow layers which can significantly save time and improve accuracy.
%Similar approaches have been put forward in the work of Furlanello \textit{et al.}~\shortcite{Author15} and Yim \textit{et al.}~\shortcite{Author16}. 
%They prove that using softmax outputs of teacher as ground truth to transfer the knowledge to student brings remarkable benefits. 
% However, previous self distillation methods transfer the individual knowledge rather than structured knowledge. 
In this work, rather than directly transferring of individual knowledge, we mainly focus on a better knowledge expression on transferring structured relation in feature space.

% \subsection{Relational Knowledge Distillation}
\paragraph{Relational Knowledge Distillation}

It’s challenging for knowledge distillation including self distillation to capture the structured information of features during distillation. This is one of the most hot topics in computer vision~\cite{Alpher07,Author17,Author18}. Notably, Chen \textit{et al.}~\shortcite{Author17} propose to transfer similarity in metric space between images using a rank loss. Park \textit{et al.}~\shortcite{Alpher07} propose relational knowledge distillation which applies $L_2$ norm function to calculate the relation of features. They demonstrate that transferring structured relation of outputs rather than individual outputs can present better understanding of knowledge. Tung \textit{et al.}~\shortcite{Author18} introduce the pairwise activation similarity within each input mini-batch to supervise the training of a student network with a trained teacher network. 
Different from previous works, we design the trainable relation networks to capture and reinforce relation of structured input data and then transfer the relational knowledge from the deepest layer to shallow layers, making better inter-class contrastiveness and intra-class similarity.


==> chapters/related_worksv1.tex <==
\section{Related Works}
Knowledge distillation is one of the most effective methods for model compression and acceleration. Breiman and Shang~\cite{Author12} first propose to train a single tree model to approximate the performance of multiple tree models.
Based on this method, Hinton \textit{et al.}~\cite{Author10} further propose the concept of knowledge distillation, known as teacher-student distillation and introduce a hyper-parameter, temperature, to control the training of student models. Many subsequent works have presented various approaches for knowledge distillation. FitNet~\cite{Author08} is put forward with the concept of hint learning to reduce the distance between feature maps of students and teachers. 
Zagoruyko \textit{et al.}~\cite{Author09} apply feature distillation on the attention map of neural networks across different layers to achieve higher accuracy. 
% Shen \textit{et al.}~\cite{Author13} propose to combine adversarial learning with knowledge distillation to minimize the differences between features of students and teachers. 
Lately, some works are proposed to solve task-specific distillation, such as semantic segmentation~\cite{SKD}, object detection~\cite{detKD} and image super-resolution~\cite{srKD}.
% Zagoruyko \textit{et al.}~\cite{Author09} apply feature distillation on the attention map of neural networks across different layers to achieve higher accuracy. 

\paragraph{Self Distillation}

Recently, a number of works~\cite{Author14,BornAgain,Author16} have shown that distilling a teacher model into a student model of identical architecture can improve the student performance to even surpass the teacher. Zhang \textit{et al.}~\cite{Author11} has proved that 
%from the perspective of generalized distillation~\cite{GeneralizedKD}, 
the features of shallow layers can be viewed as privileged information and distilling knowledge from deeper layers to shallower layers within one model can bring more accurate knowledge transferring.
This motivates us to adopt SD to address the inaccurate relational knowledge transferring due to architecture divergence, which significantly benefits accuracy boosting and time saving.
% The idea of self distillation first comes from Zhang \textit{et al.}~\cite{Author11}, where a one-step self distillation framework is proposed. 
% The key point is to transfer the knowledge from deep layers to the shallow layers which can significantly save time and improve accuracy.
% In this work, rather than directly transferring of individual knowledge, we mainly focus on a better knowledge expression on transferring structured relation in feature space.

\paragraph{Relational Knowledge Distillation}

It’s challenging for knowledge distillation including self distillation to capture the structured information of features during distillation~\cite{Alpher07,Author17,Author18}. Notably, Chen \textit{et al.}~\cite{Author17} propose to transfer similarity in metric space between images using a rank loss. Park \textit{et al.}~\cite{Alpher07} propose relational distillation which
%relational knowledge distillation which 
applies $L_2$ norm function to calculate the relation of features. They demonstrate that transferring structured relation rather than individual outputs can present better understanding of knowledge. Tung \textit{et al.}~\cite{Author18} introduce the pairwise activation similarity within each input mini-batch to supervise the training of a student network with a trained teacher network. 
Different from previous works, we design the \textit{trainable relation networks} to capture and reinforce relation of structured input data and then transfer the relational knowledge from the deepest layer to shallow layers within one model, forming better inter-class contrastiveness and intra-class similarity abstraction.


==> images/figure1.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{images/src/figure1.pdf}
\end{center}
   \caption{Overview of results on CIFAR100.}
\label{fig:results_overview}
%\label{fig:onecol}
\end{figure}

==> tabs/cifar10_results.tex <==
\begin{table}[t!]
\setlength\tabcolsep{6pt}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllllc}
\toprule
\textbf{Model} & \textbf{Baseline} & \textbf{KD} & \textbf{FitNet} & \textbf{DML} & \textbf{RKD} &\textbf{SD} & \textbf{TORSD}\\
\midrule
ResNet18 & 94.25 & 94.67 &95.57& 95.19 &95.28 & 
95.87 & $\textbf{96.38}_{\color{cGreen}{~\uparrow\textbf{2.13}}}$\\

ResNet50 & 94.69 & 94.56 &95.83&95.73&95.70&
96.01& $\textbf{96.70}_{\color{cGreen}{~\uparrow\textbf{2.01}}}$\\

ResNet101 & 94.91 & 95.23&96.01&95.73&95.97& 96.36 & $\textbf{96.93}_{\color{cGreen}{~\uparrow\textbf{2.02}}}$\\

ResNet152&94.98	&95.29	&96.10	&95.82	&96.01&96.58 & 
$\textbf{97.06}_{\color{cGreen}{~\uparrow\textbf{2.08}}}$\\

ResNeXt50-4&94.49	&95.41	&95.78	&95.41	&95.56& 96.01 & $\textbf{96.59}_{\color{cGreen}{~\uparrow\textbf{2.10}}}$\\

ResNeXt101-8&95.35	&96.38	&96.65	&96.35	&96.41&96.98& 
$\textbf{97.47}_{\color{cGreen}{~\uparrow\textbf{2.12}}}$\\

WideResNet50-2&95.18	&96.25	&96.47	&96.15
&96.27& 96.81 & $\textbf{97.03}_{\color{cGreen}{~\uparrow\textbf{1.85}}}$\\

WideResNet101-2 & 95.23	&96.27	&96.51	&96.21	&96.35
&96.89 & $\textbf{97.05}_{\color{cGreen}{~\uparrow\textbf{1.82}}}$\\

SEResNet18&94.78	&94.53	&95.64	&95.37& 95.80 & 95.51 & $\textbf{96.30}_{\color{cGreen}{~\uparrow\textbf{1.52}}}$\\

SEResNet50&94.83	&94.80	&95.31	&94.83&95.88&95.45& $\textbf{96.49}_{\color{cGreen}{~\uparrow\textbf{1.66}}}$\\

PreactResNet18&94.20 &93.74	&95.22	&94.80 & 95.21 & 95.08 & $\textbf{95.95}_{\color{cGreen}{~\uparrow\textbf{1.75}}}$\\

PreactResNet50&94.39	&93.53	&94.98	&95.87&95.53& 95.82 & $\textbf{96.49}_{\color{cGreen}{~\uparrow\textbf{2.10}}}$\\

MobileNetV1&90.16	&91.70	&90.53	&91.65	&91.52 & 91.98 & $\textbf{92.07}_{\color{cGreen}{~\uparrow\textbf{1.91}}}$\\
\midrule
Average $\Delta$ & +0.00 & & & & & & \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Top-1 accuracy (\%) on CIFAR10 across 
a number of distillation methods. 
Boldface marks the best performing accuracy.\label{2}}
\end{table}
